Our fingerprints don't fade from the Apps we touch: Fingerprinting the Android WebView

Numerous studies demonstrated that browser fingerprinting is detrimental to users' security and privacy. However, little is known about the effects of browser fingerprinting on Android hybrid apps -- where a stripped-down Chromium browser is integrated into an app. These apps expand the attack surface by employing two-way communication between native apps and the web. This paper studies the impact of browser fingerprinting on these embedded browsers. To this end, we instrument the Android framework to record and extract information leveraged for fingerprinting. We study over 20,000 apps, including the most popular apps from the Google play store. We exemplify security flaws and severe information leaks in popular apps like Instagram. Our study reveals that fingerprints in hybrid apps potentially contain account-specific and device-specific information that identifies users across multiple devices uniquely. Besides, our results show that the hybrid app browser does not always adhere to standard browser-specific privacy policies.

==> sections/rq2.tex <==
% \subsubsection*{Unique UUID in shopping apps}

% From our dataset, we observe that shopping apps add information of unique users to the user-agent strings. We show the list of apps and their fingerprints in \Cref{table:unique-uuid}.

% \begin{table}
% \centering
% \begin{tabular}{|l|l|p{0.6\linewidth}|}
%     \hline
%     Packages & Category & User Agents \\ \hline \hline
%     com.oddm.adpick & Office & Mozilla/5.0 (Linux; Android 10; Android SDK built for x86 Build/QSR1.210802.001; wv) AppleWebKit/537.36 (KHTML, like Gecko) Version/4.0 Chrome/74.0.3729.185 Mobile Safari/537.36 AdpickEncrypted:GDPViCyiXnbcQgWnvAmIBusjAV43FvgP eaw c/Xc5ayQW0rBy/oA8BUz4Vdmy9ITgwRQDnaI7 Bm ZB\#nXG5+MzNecK3HyqXv7P5/2u9yqMmkw rA/ leTfsNeUZbmjvzj9D9mECLyuBwl3lA8Sz2dt4Ue1H1t T\#n4mWgFssSh2n/eR1qpgnGRhc1cB2jqXtWuT W/cNQC\#n \\ \hline

%  net.giosis.shopping.id &
%  Shopping & 
%  \lstinline[breaklines=true]|Mozilla/5.0 (Linux; Android 11; Android SDK built for x86 Build/RSR1.210210.001.A1; wv) AppleWebKit/537.36 (KHTML, like Gecko) Version/4.0 Chrome/83.0.4103.106 Mobile Safari/537.36 Android_Gmarket Qoo10 ID_3.6.2_133(GMKTV2_ZlRnG1XAIzgwoC3OBe0hNjV4PfmyaC5R AIBqY+mkcipUGsSIiB19AyfIHQY1msEafG/xGz9RIS4=;Android SDK built for x86;11;en_US;2000010476)| \\ \hline
 
%  net.giosis.shopping.cn.nonepush &
% Shopping &
% \lstinline[breaklines=true]|Mozilla/5.0 (Linux; Android 10; Android SDK built for x86 Build/QSR1.210802.001; wv) AppleWebKit/537.36 (KHTML, like Gecko) Version/4.0 Chrome/74.0.3729.185 Mobile Safari/537.36 Android_Gmarket Qoo10 CN NOPUSH_3.6.6_137(GMKTV2_/E/eowDAPJdLOH3or4b 6kUZaqiQ9445kf50bcLzkkQeoFvJmnsEzdFnnyGmoyagfCYHYKlwCW P4=;Android SDK built for x86;10;en_US;2000000134)| \\ \hline

% Net.giosis.shopping.sg & Shopping &
% \lstinline[breaklines=true]|Mozilla/5.0 (Linux; Android 10; Android SDK built for x86 Build/QSR1.210802.001; wv) AppleWebKit/537.36 (KHTML, like Gecko) Version/4.0 Chrome/74.0.3729.185 Mobile Safari/537.36 Android_Gmarket Qoo10 SG_6.5.1_269(GMKTV2_yQ+4mthiJO62KzrgMNh9rwIUgQVt5Aax6 jISAXY3h++KFBJ4DO5/YZdeiP3jYmD+hnf246qDDdk=;Android SDK built for x86;10;en_US;200007873;US;)| \\ \hline


% xyz.quube.mobile & Shopping & \\ \hline

% mobile.qoo10.qpostpro & Shopping & \\ \hline

% Com.accelainc.ihou.fr.droid & Adventure & 
% \lstinline[breaklines=true]|2NSsaFdT 60D1F74326F469CB__5DC12396C15AB57696B4A6915216 9D 1.0.1 Mozilla/5.0 (Linux; Android 10; Android SDK built for x86 Build/QSR1.210802.001; wv) AppleWebKit/537.36 (KHTML, like Gecko) Version/4.0 Chrome/74.0.3729.185 Mobile Safari/537.36| \\ \hline
% \end{tabular}
% \caption{Unique User IDs in the User-agent strings}
% \label{table:unique-uuid}
% \end{table}

% \subsubsection*{Manually Analyzed Apps}

% We manually analyzed the user-agent strings of ten apps. We show the list of apps and their fingerprints in \Cref{table:manually-analyzed-apps}. Out of these apps, four are from social category, 4 are utilities, and two are shopping apps. 




